On exact solutions, conservation laws and invariant analysis of the generalized Rosenau-Hyman equation

In this paper, the nonlinear Rosenau-Hyman equation with time dependent variable coefficients is considered for investigating its invariant properties, exact solutions and conservation laws. Using Lie classical method, we derive symmetries admitted by considered equation. Symmetry reductions are performed for each components of optimal set. Also nonclassical approach is employed on considered equation to find some additional supplementary symmetries and corresponding symmetry reductions are performed. Later three kinds of exact solutions of considered equation are presented graphically for different parameters. In addition, local conservation laws are constructed for considered equation by multiplier approach.

==> base/apalike.tex <==
% apalike.tex, version 0.99b (8-Dec-10), for btxmac 0.99i, BibTeX 0.99c,
% TeX 3.0 or later.
%
% Copyright (C) 1990, 1991, 1992, 2010 Oren Patashnik.
% Unlimited copying and redistribution of this file are permitted as long as
% it is unmodified.  Modifications (and redistribution of modified versions)
% are also permitted, but only if the resulting file is renamed.
%
% This file, apalike.tex, contains TeX macros that let you use the
% apalike bibliography style with plain TeX.  In essence, this file
% provides the TeX counterpart to apalike.sty, the LaTeX style file
% required for using the apalike bibliography style.  Please report any
% bugs (outright goofs, misfeatures, or unclear documentation) to
% biblio@tug.org.  These macros will become frozen
% shortly after BibTeX version 1.00 is released.
%
% AMS-TEX WARNING: This style (apalike) doesn't work with AmS-TeX's
% `amsppt' style, because AmS-TeX redefines the tie character `~' of
% plain TeX, and the `amsppt' style redefines plain TeX's `\nobreak'
% macro, so that a multiple-author reference for which `apalike'
% automatically produces an in-text citation like `(Jones et~al., 1992)'
% will throw AmS-TeX's `amsppt' style into an infinite loop, exceeding
% its input stack size.  (I've checked no other AmS-TeX styles for this
% problem.)  The AmS-TeX warning of btxmac.tex gives more information.
% END OF AMS-TEX WARNING.
%
% Editorial note (i.e., flame):
% Many journals require a style like `apalike', but I recommend that you
% not use it if you have a choice---use something like `plain' instead.
% Mary-Claire van Leunen (A Handbook for Scholars, Knopf, 1979) argues
% convincingly that a style like `plain' encourages better writing than
% one like `apalike'.  Furthermore the best argument for using an
% author-date style like `apalike'---that it's "the most practical"
% (The Chicago Manual of Style, University of Chicago Press, thirteenth
% edition, 1982, pages 400--401)---falls flat on its face with the new
% computer-typesetting technology.  For instance page 401 of the Chicago
% Manual anachronistically states "The chief disadvantage of [a style
% like `plain'] is that additions or deletions cannot be made after the
% manuscript is typed without changing numbers in both text references
% and list."  With (La)TeX the disadvantage obviously evaporates.
% Moreover, apalike indulges in what I think is a shortsighted practice:
% automatically abbreviating first names.  Abbreviating may occasionally
% make the work a page shorter, but at the cost of a less useful
% reference list; that's too high a cost for such a marginal benefit.
% The offense isn't egregious for a name like `Donald E. Knuth'---at
% least among those familiar with his field---since there aren't many
% other `D. E. Knuth's floating around.  But referring to `D. E. Smith'
% in a field having more than one can be quite confusing.  Moreover,
% with the proliferation of computers and citation indexes nowadays,
% it's important to indicate in the reference list an author's name
% exactly as it appears in the work cited.  Automatically abbreviating
% first names is simply bad scholarship.  (End of flame.)
%
% To use these macros you need the btxmac.tex macros, which let you use
% BibTeX with plain TeX (rather than with LaTeX); the file btxmac.tex
% explains those macros in detail, and gives examples.  You simply
% \input apalike right after you \input btxmac to invoke these macros.
%
%
%   HISTORY
%
% Oren Patashnik wrote the original version of these macros in December
% 1990, for use with btxmac.tex.
%
%   12-Dec-90  Version 0.99a, first general release.
%   29-Feb-92  0.99b, changed `\biblabelextrahang' to `\biblabelextraspace',
%                     to keep up with btxmac.tex version 0.99i.
%    8-Dec-10  Still version 0.99b, as the code itself was unchanged;
%                     this release clarified the license.
%
% Here, finally (I swear, I thought he was never gonna stop), are the
% macros.  The first bunch makes the label empty and sets 2em of
% hanging indentation (via \biblabelextraspace) for each entry.
%
\def\biblabelprint#1{\noindent}%
\def\biblabelcontents#1{}%
\def\bblhook{\biblabelextraspace = 2em }%
%
%
% And the last bunch formats an in-text citation: parens around the
% entire citation; semicolons separating individual references; and a
% comma between a reference and its note (like `page 41') if it exists.
%
\def\printcitestart{(}%         left paren
\def\printcitefinish{)}%        right parent
\def\printbetweencitations{; }% semicolon, space
\def\printcitenote#1{, #1}%     comma, space, note (if it exists)

